Where Have All the Kaczmarz Iterates Gone?

The randomized Kaczmarz (RK) algorithm is one of the most computationally and memory-efficient iterative algorithms for solving large-scale linear systems. However, practical applications often involve noisy and potentially inconsistent systems. While the convergence of RK is well understood for consistent systems, the study of RK on noisy, inconsistent linear systems is limited. This paper investigates the asymptotic behavior of RK iterates in expectation when solving noisy and inconsistent systems, addressing the locations of their limit points. We explore the roles of singular vectors of the (noisy) coefficient matrix and derive bounds on the convergence horizon, which depend on the noise levels and system characteristics. Finally, we provide extensive numerical experiments that validate our theoretical findings, offering practical insights into the algorithm's performance under realistic conditions. These results establish a deeper understanding of the RK algorithm's limitations and robustness in noisy environments, paving the way for optimized applications in real-world scientific and engineering problems.

==> ex_shared_xxx.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
% Sets running headers as well as PDF title and authors
%\title{Where Have all the Kaczmarz Iterates Gone?}{Bergou, Boucherouite, Dutta, Li, Ma}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Where Have all the Kaczmarz Iterates Gone?}

% Authors: full names plus addresses.
\author{El Houcine Bergou \thanks{College of Computing, Mohammed VI Polytechnic University, Morocco, (\email{elhoucine.bergou@um6p.ma}).}
\and
Soumia Boucherouite \thanks{College of Computing, Mohammed VI Polytechnic University, Morocco, (\email{soumia.boucherouite@um6p.ma}).}
\and 
Aritra Dutta \thanks{Department of Mathematics, University of Central Florida, USA, (\email{aritra.dutta@ucf.edu}, \url{https://sciences.ucf.edu/math/person/aritra-dutta/}).}
\and
Xin Li\thanks{Department of Mathematics, University of Central Florida, USA, (\email{xin.li@ucf.edu}).} 
\and 
Anna Ma \thanks{Department of Mathematics, University of California, Irvine, USA, (\email{anna.ma@uci.edu}).}
}
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

